Contamination Bias in Linear Regressions

We study regressions with multiple treatments and a set of controls that is flexible enough to purge omitted variable bias. We show that these regressions generally fail to estimate convex averages of heterogeneous treatment effects -- instead, estimates of each treatment's effect are contaminated by non-convex averages of the effects of other treatments. We discuss three estimation approaches that avoid such contamination bias, including the targeting of easiest-to-estimate weighted average effects. A re-analysis of nine empirical applications finds economically and statistically meaningful contamination bias in observational studies; contamination bias in experimental studies is more limited due to smaller variability in propensity scores.

==> starB.tex <==
Small &  & 0.155 & -0.204 & 0.062 & -0.220\\
 &  & (0.160) & (0.220) & (0.135) & (0.194)\\
Aide &  & -0.183 & 0.107 & -0.086 & 0.166\\
 &  & (0.149) & (0.188) & (0.125) & (0.194)

